Contention Resolution with Predictions

In this paper, we consider contention resolution algorithms that are augmented with predictions about the network. We begin by studying the natural setup in which the algorithm is provided a distribution defined over the possible network sizes that predicts the likelihood of each size occurring. The goal is to leverage the predictive power of this distribution to improve on worst-case time complexity bounds. Using a novel connection between contention resolution and information theory, we prove lower bounds on the expected time complexity with respect to the Shannon entropy of the corresponding network size random variable, for both the collision detection and no collision detection assumptions. We then analyze upper bounds for these settings, assuming now that the distribution provided as input might differ from the actual distribution generating network sizes. We express their performance with respect to both entropy and the statistical divergence between the two distributions -- allowing us to quantify the cost of poor predictions. Finally, we turn our attention to the related perfect advice setting, parameterized with a length $b\geq 0$, in which all active processes in a given execution are provided the best possible $b$ bits of information about their network. We provide tight bounds on the speed-up possible with respect to $b$ for deterministic and randomized algorithms, with and without collision detection. These bounds provide a fundamental limit on the maximum power that can be provided by any predictive model with a bounded output size.

==> olderbounds.tex <==

\section*{Older Lower Bound Material to be Selectively Integrated into Main Body of Paper}



Let us start with a simple setup for studying the impact of advice on contention resolution.
Imagine that a protocol now includes: (a) a process for each player from set $P$ of $n$ possible players; and (b) and an advice
function $f:P\rightarrow \{0,1\}^b$, that provides $b$ bits of {\em advice} to the players about the target set.
An execution unfolds as follows. 
First, an adversary chooses a non-empty {\em target set} $T \subseteq P$.
Second, each player in $T$ is activated and provided $f(T)$ as additional input.
These players now execute their processes with the input $f(T)$. The problem
is solved the first round a player transmits alone.
We call this combination of $f$ and the process definitions a {\em $b$-advice protocol}.

The key question here is to quantify the degree to which bits of advice can help speed up this problem.
We know, for example, that for $b\geq \log{n}$, the problem can be trivially solved with an advice
function that simple returns the id if a player in $T$.
But what about smaller $b$? For $1 \leq b < \log{n}$, what is the best possible speed up, and what strategy
obtains it?





\subsection{An $\Omega(\frac{\log^2{n}}{2^b})$ Round Lower Bound for $b$ Bits of Advice, High Probability, and No CD}
Let us consider the classic case of no collision detection and an algorithm that needs to solve
the problem with with high probability in $n$.
Let $t_{opt}(n)$ be the optimal time complexity for solving this problem with for a given $n$.
That is, for each $n>1$, every algorithm needs at least $t_{opt}(n)$ rounds to solve the problem with probability at least $1-1/n$.
We know that $t_{opt}(n) \geq \alpha \log^2{n}$, for some constant $\alpha$.

Here is a key claim for which I will sketch a proof:

\begin{theorem}
Let ${\cal A}$ be a $b$-advice protocol,
for some $b\geq 0$, 
that guarantees for every $n>1$ and no collision detection,
to solve contention resolution in at most $t_b(n)$ rounds with probability at least $1-1/n$.
It follows:

\[ t_b(n) \geq \frac{t_{opt}(n)}{2^b} = \Omega\left( \frac{\log^2{n}}{2^b} \right). \]
\end{theorem}
\begin{proofsketch}
We begin by replicating some definitions and claims used from the lower bound proof 
for this setting with no advice.
In particular, fix some count $x>1$
and let $[x] = \{1,2,...,x\}$.
In the earlier paper, we
established that there exists a sequence $Q_x$,
made up of subsets of $[x]$,
such that: (1) $|Q_x| \leq c_1 x^8$, for some constant $c_1 > 0$;
and (2) it takes at least $t_x = c_2 \log^2{x}$ subsets of $[x]$
to {\em hit}\footnote{Intersect at exactly one element} 
every set in $Q_x$, for some other constant $c_2 > 0$.

Fix some player count $n_x = |Q_x| + 1$.
Consider an adversary for the no advice setting for this $n_x$
that chooses its target set with uniform randomness from $Q_x$.
(Notice, this adversary is restricted, as it is ignoring all ids between
$x+1$ and $n_x$. But this only makes the player's job even easier,
therefore strengthening any lower bound argument.)

The key observation from the original proof for this setting
is that if a contention resolution protocol runs for strictly
less than $t_x$ rounds, then it missed at least one set from $Q_x$.
The probability that the adversary happened to select
that set was is $1/|Q_x| = 1/(n-1) > 1/n$, meaning its failure
probability is too large.
In this summary of the argument, and in the below generalization,
I am skipping past some details of how you connect a contention resolution 
protocol to generating a sequence that attempts to hit $Q_x$.
The basic ``simulation strategy," however, is to just run the protocol
all all processes and use the processes that transmit in round $r$
as set $r$ in your sequence attempting to hit $Q_x$.
The details are in the original paper.

It follows that $t_x$ is a lower bound for the problem for $n_x$.
Because $t_x = c_2 \log^2{x}$ can be expressed as $c_2 \log^2{(n^{1/8}c_3 )}$,
for some constant fraction $c_3>0$,
we get a lower bound in $\Omega(\log^2{n})$.

We now use these same definitions and claims for our new lower bound for the $b$-advice
setting.
Fix a $b$-advice protocol ${\cal A}$ with advice function $f$.
For the sake of this lower bound,
we will restrict the adversary to only selecting target sets from $Q_x$,
so we will consider only those sets in the following.

For each advice string $s\in \{0,1\}^b$,
let $T(s) = \{ T \in Q_x:  f(T) = s\}$ contain all the target sets (if any) from $Q_x$ that generate advice $s$.
Notice for every subset $T$ of $[x]$,
there is some advice string $s$ such that $T\in T(s)$;
namely, $s=f(T)$.
Also for each such $s$,
 let $\ell(s)$ be a minimum length sequence of subsets of $[x]$ that {\em hits}
every set in $T(s)$. 
Let $\ell^* = \max_{s\in \{0,1\}^b}\{\ell(s)\}$.
We consider two cases for $\ell^*$.


\begin{itemize}



    \item {\em Case $1$:} $\ell^* < t_x/2^b$.

Consider the sequence $H$ that results from appending together $\ell(s)$,
for each $s\in \{0,1\}^b$.
As we argued above, every set in $Q_x$ is hit by some $\ell(s)$,
so $H$ hits every set in $Q_x$.
By construction, however, $|H| < \ell^* \cdot 2^b < t_x$.
This contradicts the above claim that any set that hits all of $Q_x$ 
must be of length at least $t_x$.



\item {\em Case $2$:} $\ell^* \geq t_x/2^b$.

By the definition of $\ell^*$,
in this case there must exist some advice string $s\in \{0,1\}^b$
such that $\ell(s) \geq t_x/2^b$.
Consider an adversary that chooses a target set with uniform randomness from $T(s)$.

Assume for contradiction that our fixed $b$-advice protocol ${\cal A}$
guarantees to solve contention resolution with high probability in strictly
less than $\ell(s)$ rounds.
It follows, as in our original no advice setting proof, 
that in these many rounds ${\cal A}$ will fail to hit at least one set in $T(s)$.
With probability $1/|T(s)| \geq 1/|Q_x| = 1/(n-1)$,
the adversary will have chosen the set that is missed.
This contradicts the assumption that ${\cal A}$ fails with probability at most $1/n$
when run for this duration.

\end{itemize}


Pulling together the pieces, we just
proved that if ${\cal A}$ guarantees to solve the problem in $q(n)$ rounds with probability at least $1-1/n$,
then regardless of the definition of its advice function, it must be the case that $q(n) \geq t_x/2^b$ rounds.
As in our the original argument from the no advice setting,
we note that $t_x = c_2 \log^2{(n_x^{1/8}c_3 )}$, for the appropriate constants $c_2$ and $c_3$,
and therefore this bound is in $\Omega(\log^2{n}/2^b)$, as claimed.
\end{proofsketch}

\paragraph{A General Upper Bound Strategy}

Fix a sequence $Q$ of subsets of $[n]$ that guarantee
to hit any target set $T\subseteq [n]$.
We know that $|Q| \in \Omega(\log^2{n})$.

We can use $Q$ as the foundation of a $b$-advice protocol as follows.
Build a binary tree where the leaves correspond to the sets in $Q$.
For each target set $T\subseteq [n]$,
let $Q(T)$ be a set from $Q$ that hits $T$.
Define the advice function $f(T)$
to encode the first $b$ steps in a traversal of our tree from the root toward the $Q(T)$ leaf
(i.e., 0 means descend to the left subtree and 1 means descend to the right).

We can now define a natural protocol to use $f$.
Given advice $s$,
descend through the tree $|s|$ steps, to 
arrive at a subtree.
Now simply ``try" the leaves of this subtree in order (to try a given set simply means you broadcast in the round
if and only if you are in the set).

If we had some $Q$ near the minimal length---e.g., $|Q| = O(\log^2{n})$---then we would have
an optimal algorithm.
Given $b$ bits of advice, we reduce the original set of $\approx \log^2{n}$ sets to try
by multiplicative factor of $1/2^b$, arriving at an optimal $O(1)$ solution once we get near
$b=2\log\log{n}$.

Alas, no such sequence near optimal exists.
In the formal terminology of selector theory,
such a $Q$ would provide an {\em $(n,n)$-selective family}.
The best known existential bounds for such families is of size $\Omega(n)$,
and this bound is tight.\footnote{\url{http://people.csail.mit.edu/cnewport/bibs/selectors.shtml}}.
We must actually deploy randomness to get closer to our lower bound.

\paragraph{A Tight Upper Bound for Strong Shared Randomness.}
Let us identify some set of assumptions under which a tight bound is possible.
Consider shared randomness. Assume further that the advice function also knows this shared randomness
This is a strong assumption. Notice, however, that our lower bound still holds under this assumption

Here is our strategy.
All nodes begin by locally simulating a standard $O(\log^2{n})$ round high probability solution
to contention resolution, such as the {\em decay} routine, being run on all $n$ nodes.
In particular, assume $t = c\log^2{n}$ rounds, for some constant $c>0$, is enough to ensure the strategy
will solve the problem with high probability.
For each round $r$ of the simulation, let $S_r$ be the nodes that transmit.
Let $Q$ be the whole sequence $\langle S_1, S_2, ..., S_t\rangle$.
All nodes run the simulation using shared randomness so they all learn thee same $Q$.
Crucially, because we assume $f$ has these bits, it too can be defined with respect to $Q$.

Imagine a (nearly) balanced binary tree with one leaf or each set in $Q$.
Under the assumption that $Q$ solves contention resolution,
at least one leaf is associated with a set $H$ that solves the problem for the target $T$ in question.
The advice function follows the general strategy outlined above and returns the first $b$ steps
in a traversal in the tree from the root down to $T$.
Each step down the number of leaves in contention by a factor of $2$,
leaving nodes with only $|Q|/2^b = O(\log^2{n}/2^b)$ leaves to iterate through to solve the problem.

\paragraph{Toward a Tight Bound Without Shared Randomness (but a Randomized Knowledge Function).}
Here we seek if it is possible to get an constant round solution with $O(\log\log{n})$ bits of advice,
matching the lower bound at least for the large values of knowledge.
The solution sketched here is not complete. It requires that the knowledge function can generate random
bits, but that there is no shared randomness.
We will begin with strong assumptions that yield a straightforward answer, and then work to increasingly remove these assumptiomns
at the cost of more complexity.

Let us begin with the following strong assumption. The adversary can select the number of participants, $k$, but then the ids are of these participants are each generated from scratch by flipping $\log{n}$ independent fair coins for each to generate a $\log{n}$-bit id.
These are then the specific $k$ participants activated.

For a given $k$, we expect a constant number of participants to have an id that begins with the pattern $1^{\log{k}}$
(this is true, of course, for any fixed prefix of $\log{k}$ bits.
If we consider a conservative target value of $t_k = \lfloor \log{k} - \log\log{n} \rfloor$,
the expected number of participants with an id that begins with $1^{t_k}$ is now:

\[ k / 2^{t_k} = k / 2^{ \log{k} - \log\log{n} } = k / 2^{ \log{k/\log{n}} }= \log{n}. \]

This calculation only works assuming that $\log{k} > \log\log{n}$ which implies $k \in \Omega(\log{n})$.
Put aside for now the case of smaller $k$ as we can solve that case more directly.

If we play with the constants in $t_k$, 
then we can get a guarantee that the number of participants with ids that begin with $1^{t_k}$
is $\Theta(\log{n})$, with high probability in $n$.
If $k$ is sufficient larger than $\log{n}$, therefore,
our advice function can use $\log\log{n}$
bits to specific $t_k$ by specify the relevant $t_k$,
as it can only take $\log{n}$ values.

At this point, only participants whose ids begin with $1^{tk}$
continue. We have reduced the number of participants to strictly
greater than $1$ and no more than $O(\log{n})$.
If $k$ is too small for the above analysis to go through,
we can just skip this first phase as that means we {\em began}
with a number of participants between $1$ and $\log{n}$,
with no further reductions required.

At this point, we have reduced the participants in a way that the
knowledge function {\em knows} which participants remain.
This latter part is crucial and why we cannot use simpler randomized
techniques among the participants themselves to reduce their numbers.
Let $k'$ be this reduced number.

Now our goal is to isolate a single node in a constant number of rounds with
just an additional $O(\log\log{n})$ bits
Here the key is to turn to a combinatorial object known
as a $(n,k')$-selective family.
We can construct a sequence ${\cal Z}$ of no more than a polylogarithmic 
subsets of $[n]$ such that we guarantee for any subset of $[n]$
of size no more than $k'$,
there is some set in ${\cal Z}$ that intersects it at exactly one id.
We can use $O(\log{|{\cal Z}|}) = O(\log\log{n})$ more bits to 
specify the set in ${\cal Z}$ that creates this intersection and wins the game.

Now we need to remove our assumption of randomly generated ids for the participants.
One idea is to allow the advice function to generate a random {\em mask}
of $\log{n}$ bits, each generated with independent uniform randomness, which is
then sent to the participants who apply it to their ids to get re-randomized ids.

I am not sure yet that this is enough, but let us assume for now it is.
We still have not solved our problem because if the advice function sends $\log{n}$
bits it might as well specify an id of a participant and solve the problem directly.
Here, however, we can apply pseudorandomness theory to show that the advice function
only need send a random $O(\log\log{n})$-bit seed which can be expanded to $\log{n}$
bits in a way that is similarly random.

(In particular, see the generalization of Newman's Theorem from my PODC 2016 paper.
The basic idea is that there exists a set of poly-log masks such that
if we randomly choose one from that set it is similar to generate a mask
from scratch. It takes $\log\log{n}$ bits to specify a selection from a set
of  polylog size.)

{\em Not so fast!} The above does not quite work as for sufficiently small $t_k$,
the adversary will just choose $k$ participants so that they all have the
same prefix for the first $t_k$ bits, meaning that random masks will have a uniform effect on them.
Here are a few proposals for how to get around this issue:

\begin{itemize}
    \item Have the advice function specify two values of size $\log\log{n}$:
    the starting point of the mask and its duration; e.g., the pair $(i,j)$
    means that we are selecting for participants whose ids have $j$ $1$ bits
    in a row starting at position $i$ (and wrapping around, if needed).
    
    \item Have the advice function send a random seed to be combined with
    each nodes full id to generate a string of nearly independent random
    bits for each node to use as a mask; that would get us back closer
    to where we need to be.
    
\end{itemize}


\subsection{An $\Omega(\frac{\log{n}}{2^b})$ Round Lower Bound for $b$ Bits of Advice, Constant Probability, and No CD}

In the no advice setting, shifting from high probability to constant probability reduced the lower bound
from $\Omega(\log^2{n})$ to $\Omega(\log{n})$. Here we claim a similar log factor improvement
occurs in the presence of $b$ bits of advice.

\begin{theorem}
Let ${\cal A}$ be a $b$-advice protocol,
for some $b \geq 0$,
that guarantees for every $n>1$ and no collision detection,
to solve contention resolution in at most $t_b(n)$ rounds with probability at least $1/2$.
It follows:

\[ t_b(n) \in \Omega\left( \frac{\log{n}}{2^b} \right). \]
\end{theorem}
\begin{proofsketch}
The same argument used for the high probability case should still more or less
work. Now, for each advice string $s$, have $\ell(s)$ describe the minimum length string to cover
at least half of the sets in $T(s)$, and let $\ell^*$ once again be the maximum of these minimums 
over all advice strings.

As before, if $\ell^* < c\log{n}/2^b$,
then we can append the $\ell(s)$ strings to get a sequence that hits all the set in less than $c\log{n}$
rounds. For a sufficiently small constant fraction $c$, however, this contradicts a combinatorial bound
from no advice setting paper.

On the other hand, if there is some $s$ where $\ell(s) \geq c\log{n}/2^b$,
 we can, as before, have the adversary pick a set from $T(s)$.
 If we run the protocol for less than $c\log{n}/2^b$ rounds,
 then half or more of the sets are uncovered, and with probability greater than
 $1/2$, the adversary selected one of the uncovered sets.
\end{proofsketch}

\paragraph{Notes on a Matching Upper Bound}
In this case, a matching upper bound seems straightforward.
Consider the $\log{n}$ guesses $S =\{1,2,4,8,...,n\}$.
If you provide a contention resolution protocol that guess $q\in S$ that is closest
to the actual number of participants, $k$, then we can solve the problem in one round
with constant probability by having all participants transmit with probability $1/q$.
If we do this a constant number of times, for a sufficiently large constant, we can
drive the failure probability below $1/2$.

With this in mind, consider a $b$-advice protocol in which we
fix a balanced binary tree with one leaf for each of the $\log{n}$ values in $S$.
The advice encodes a descent toward a leaf in this tree, with a $0$ meaning descend to the left
sub-tree and a $1$ meaning descend to the right sub-tree.
Let $q^* \in P$ be the {\em target} value closest to the actual number of participants.
The advice function encodes in its advance the first $b$ steps in a descent from
the root to the leaf corresponding to $q^*$.

For $b \geq \log\log{n}$, 
the advice function can specify $q^*$ exactly. By our above argument, the nodes in the protocol
can then drive their failure probability down below $1/2$ in $O(1)$ rounds of transmissions.
For $b< \log\log{n}$,
the nodes cycle through the only the values corresponding to the leaves
of the sub-tree that the advice descends to in the tree.
There are $\log{n}/2^b$ such leaves, so $O(\log{n}/2^b)$ rounds are sufficient
to solve the problem with probability at least $1/2$.



\subsection{An $\Omega(\frac{\log{n}}{2^b})$ Round Lower Bound for $b$ Bits of Advice, High Probability, and CD}

Let us now consider the case with collision detection.
With no advice the relevant lower bound is $\Omega(\log{n})$ rounds.
Indeed, this bound is shown to hold for the easier case in which the protocol is guaranteed
that the number of participants is always exactly $2$. 
This bound is tight as with collision detection you can solve this problem deterministically for
any number of participants in $O(\log{n})$ rounds.
This algorithm works by assuming a binary tree with one leaf for each of the $n$ possible participants.
The participants can use collisions to {\em vote} for descending to the left or right sub-tree,
and by doing so, descend together to the node corresponding to participant with the smallest id.

We can use as similar argument as for the no collision detector cases to establish
that $b$ bits of advice gives you at most a $2^b$ factor speed up.

\begin{theorem}
Let ${\cal A}$ be a $b$-advice protocol,
for some $b \geq 0$,
that guarantees for every $n>1$ and  collision detection,
to solve contention resolution in at most $t_b(n)$ rounds with high probability.
It follows:

\[ t_b(n) \in \Omega\left( \frac{\log{n}}{2^b} \right). \]
\end{theorem}
\begin{proofsketch}
The proof for the no advice setting followed the same general structure as the two cases we have
studied so far for no collision detector.
The underlying combinatorial claim in this case 
is straightforward to establish than those used for the other cases. 
Fix any $k>1$,
and consider the set $P_k = \{(i,j)| i,j \in [k]\}$ of all pairs.
A simple counting argument establishes that you need at least $\log{k}$ sets
to guarantee to hit pairs in $P_k$.
If we set $k$ to $cn^{1/2}$, for a sufficiently small constant $c$,
then $|P_k| < n$.
It follows that in less that in less $\log{k} = \Omega(\log{n})$ rounds,
you leave at least one pair $(i,j)$ not hit.
If the adversary chooses the target with uniform randomness,
it selects this bad target with probability $1/|P_k| > 1/n$.

We can now once again apply our same bucket argument from the previous
advice cases.
If every bucket has {\em fast} sequence that hits all pairs in the bucket,
then we can append them to get a sequence that hits all pairs in {\em fast},
contradicting our combinatorial property from above.
If at least one bucket requires $\Omega(\log{n}/2^b)$,
we can then just focus on that bucket to obtain the lower bound---if a protocol
leaves a set uncovered, we select that set with probability greater than $1/n$.
\end{proofsketch}

\paragraph{A Matching Upper Bound for the Restricted Case of $2$ Nodes.}

As in the no advice setting, our lower bound holds for the easier case
where the number of participants is guaranteed to be limited to $2$.
In that case, we can easily match the lower bound of $\Omega(\log{n}/2^b)$.
Imagine a binary tree with one leaf for each of the $\log{n}$ bit positions
in the node ids.
The advice function's advice descends in the tree toward the the first bit
that differs between the two participants.
Descending $b\leq \log\log{n}$ steps in the tree brings the two players to
a sub-tree with only $\log{n}/2^b$ leaves. They can then cycle through
those leaves from left to right: for each, only transmitting if they
have a $1$ in that bit position of their id.

\paragraph{On Upper Bounds for General Number of Participants.}
Unlike in the no advice setting, the problem seems harder when
there can be any number of participants.

\subsection{Deterministic Lower Bounds}

In a December meeting, Alex sketched how to generalized the rectangle approach used in classical communication complexity
results to show that a small amount of advice cannot help you deterministicly reduce contention.
To be more concrete, let us start with a simple version of the problem called {\bf \em $f(n)$-non-interactive contention resolution}.
In this version of the problem, the participants do not communicate on a shared channel. They just make individual decision
about whether or not they are a leader based only on their id and any advice they receive. 
We say a strategy solves the problem for a given $f(n)$ if no more than $f(n)$ participants declare themselves leader.

I believe what Alex proved was something like the following:

Note the reference used below is \href{https://reader.elsevier.com/reader/sd/pii/S0304397502008514?token=45F3454E5F8B28E539571F6DDC2188D477331ADD40B7FE55A967938D9C174BD0542A42BB921CDAA6FB30496AB8817157}{\texttt{here}}

\begin{theorem}

Any deterministic algorithm which has an active node broadcast alone in a single round after the advice is received must use at least $\log{n}-O(1)$ bits of advice.
\label{thm:noninteractive}
\end{theorem}

\begin{proof}

Fix some set of active nodes $V_A\subseteq V$ and some advice string $s$. In the non-interactive single-round setting, the advice string $s$ must solidify the decision for each node of whether or not to broadcast. Let $V(s)\subseteq V$ be the subset of nodes which decide to broadcast based on receiving $s$. Notice that all we require is that $|V(s)\cap V_A|=1$ and so it's not necessary that $V(s)\subseteq V_A$. In other words, $s$ may also instruct some inactive nodes to broadcast (allowing the algorithm to \textit{reuse} advice in the case that these nodes are active).

\par

If $S$ is the set of all possible advice strings, let $\mathcal{F}=\{V(s)\mid s\in S\}$ be the set of all subsets of nodes that are instructed to broadcast given each different advice string. In order for an algorithm to guarantee that one node broadcasts alone, it must be the case that for every subset $V_A\subseteq V$, there must exist some $s$ such that $V(s)\subseteq \mathcal{F}$ and $|V(s)\cap V_A|=1$. In other words, $\mathcal{F}$ must constitute an $(n,n)$-selective family.

\par

Given $b$ bits of advice, we know that $|\mathcal{F}|=2^b$. From \cite{clementi:2002} we have that for any $(n,n)$-selective family $\mathcal{F}$, $|\mathcal{F}|\geq n/c$ for some constant $c$. Therefore $2^b\geq n/c$, such that $b\geq \log{n}-\log{c}$. Stated another way, if our algorithm could solve the problem with fewer than $\log{n}-\log{c}$ bits of advice, the set of corresponding subsets would constitute a selective family with fewer than $n/c$ subsets, which contradicts the result from \cite{clementi:2002}. Therefore at least $\log{n}-\log{c}=\log{n}-O(1)$ bits of advice are required.


\end{proof}


% \begin{theorem}
% There exists a bound $\ell_1 = \Omega(\log{n})$ such that for every advice function $f_{adv}$ that returns no more than $\ell_1$
% bits of advice, there is no deterministic algorithm that solves $1$-non-interactive contention resolution with $f_{adv}$.
% \label{thm:noninteractive}
% \end{theorem}

This is a strong bound because, of course, for $\ell_1 = \log{n}$, the problem is trivially solvable as the advice function
can simply return the id of one of the participants. The implication is that deterministic solutions cannot do much better than
the trivial advice solution.
We will now build on the above bound---which I hope I remembered right---to get additional results.

\paragraph{Lower Bounds for $O(\text{polylog}(n))$-Non-Interactive Contention Resolution.}
Consider, now, an advice function that would allow a set of participants to deterministically
reduce their numbers down to no more than $O(\text{polylog}(n))$.
This also requires at least $\ell_2 = \Omega(\log{n})$ bits of advice, albeit for an $\ell_2 < \ell_1$.
In more detail:

\begin{theorem}
There exists a bound $\ell_2 = \ell_1 - O(\log\log{n}) = \Omega(\log{n})$, such that for every advice function $f_{adv}$ that returns no more than $\ell_2$
bits of advice, there is no deterministic algorithm that solves $O(\text{polylog}(n))$-non-interactive contention resolution with $f_{adv}$.
\label{thm:noninteractive2}
\end{theorem}

To get this result, notice that if there are only $k=O(\text{polylog}(n))$ participants, and $k$ is known,
we can solve the problem 
with $O(\log\log{n})$ bits of advice. All players can agree in advance on an $(n,k)$-selective family
of size $O(k\log{n}) = O(\text{polylog}(n))$.
One the advice function sees the actual set of participants, it can use $O(\log\log{n})$ bits
to identify which set from this selective family isolates a node from this participant set.
The participants broadcast if and only if they are in that set---solving the problem.

Now assume you can deterministically and non-interactively
reduce to no more than $k$ nodes with $\ell_2$ bits of advice.
Because the strategy is deterministic, the advice function knows which $k$ nodes will
service. It can then append an extra $O(\log\log{n})$ bits to its advice to further identify
a single winner. 
Therefore, $\ell_2 + O(\log\log{n})$ bits would be suffificient, meaning that $\ell_2$ cannot be too much smaller
than the $\ell_1$ bound from Theorem~\ref{thm:noninteractive}.


\paragraph{Lower Bound for Deterministic Contention Resolution without CD.}
Here we build on Theorem~\ref{thm:noninteractive} to prove a lower bound
for the advice required for general deterministic solutions to the contention resolution problem.
The problem can be trivially solved in one round given $\log{n}$ bits of advice.
We show that as we reduce this advice to 
$\alpha\log{n}$ bits, for some  fraction $\alpha < 1$,
the rounds required grow roughly as $n^{1-\alpha}$,
We will then show this is tight within constant factors.

\begin{theorem}
Assume that $A$ is deterministic solution to contention resolution and $f$ is an advice function
such that $A$ can solve contention resolution in $t(n)$ rounds given  no more than $\alpha\log{n}$ bits of
advice from $f$, for some constant $\alpha<1$, in a network of size $n$ with no collision detection.
It follows that $t(n) \geq n^{1-\alpha}/c$, for some constant $c$.
\end{theorem}
\begin{proof}
Fix some $A$, $f$, $t$, $n$, and $\alpha$, as specified by the theorem.
Recall that Theorem~\ref{thm:noninteractive} tells us that deterministic non-interactive contention
resolution requires $\log{n} - b$ bits of advice, for some constant $b> 0$.

Our strategy in this proof is to deploy the advice function $f$, designed for general
contention resolution without collision detection, to create a related advice function $f'$
for the non-interactive setting.
To do so, given a participant set $P$, let $\alpha$ be the execution $\alpha$
that results when the participants in $P$ run $A$ given initial advice $f(P)$.
By assumption, the execution $\alpha$ solves contention resolution by round $r \leq t(n)$.
Crucially, because $A$ assume no collision detection, no participant in $\alpha$ receives
anything until round $r$. Therefore, each participant can simulate the first $r-1$ rounds
locally by just simulating $A$ with nothing being received.

It follows that to solve non-interaction contention resolution it is enough
to give each participant the pair $(t(P), r)$, allowing them to locally simulate $\alpha$
through the first $r-1$ rounds, and then simply execute round $r$---solving contention resolution
in one round without any interaction.
The bits required to encode this advice are upper  bounded as:
$f(P) + \lceil \log{t(n)} \rceil  \leq  \alpha\log{n} + \lceil \log(t(n)) \rceil$.

Applying our above bound on non-interactive collision detection, it follows:

\begin{eqnarray*}
%
\alpha\log{n} + \lceil \log(t(n)) \rceil & \geq & \log{n} - b \Rightarrow \\
%
\lceil \log(t(n)) \rceil & \geq & \log{n} - b - \alpha\log{n} \Rightarrow \\
%
\lceil \log(t(n)) \rceil & \geq & \log{n} - b - \alpha\log{n} \Rightarrow \\
%
 \log(t(n)) + 1 & \geq & (1-\alpha)\log{n} - b \Rightarrow \\
%
2^{ \log(t(n))}2 & \geq & 2^{(1-\alpha)\log{n}}2^{-b} \Rightarrow \\
%
2t(n) & \geq & n^{1-\alpha}2^{-b} \Rightarrow \\
%
t(n) \geq & n^{1-\alpha}/c, \\
\end{eqnarray*}

\noindent where constant $c=2^{b+1}$. This establishes our theorem.
\end{proof}


It is not hard to show that the above bound is close to tight.
Assume are restricted to $q = \alpha\log{n}$ bits of advice for some $\alpha<1$.
Assign the $n$ possible participants to the leaves of a balanced binary tree of height $\log{n}$.
Given $\log{n}$ bits of advice, it is possible to encode a traversal 
through this tree from the root down to a specific leaf, corresponding the id of a participant.
For $q<\log{n}$ bits,
we can record the first $q$ steps of such a traversal toward a participant.
Given this traversal prefix all participants can reduce the number of possible identities
of this target participant by a factor of $2$ with each step deeper into the tree.
The result is that only $n/q = n/2^{\alpha\log{n}} = n/n^{\alpha} = n^{1-\alpha}$
possible identities remain. The participants can solve the problem in an additional
$n^{1-\alpha}$ rounds by trying these remaining identities one at a time.
The resulting algorithm is within a constant factor of the bound proved above.


 
 \paragraph{Lower Bound for Deterministic Contention Resolution with CD}
 In this case, the problem can always be solved in $2\log{n}$ rounds by using
 the collision detection to descend down a binary tree with one leaf for each of the $n$ possible participants.
 There is a lower bound of $\Omega(\log{n})$ for the no-advice case (indeed, it holds even for random solutions and high probability success).
Clearly, $\log{n}$ bits of advice trivially solves the problem by identifying a single participant.
The question is whether we can solve the problem non-trivially faster than $\log{n}$ 
with non-trivially fewer than $\log{n}$ bits of advice.
Here we can establish a stronger bound, showing there is a threshold $q = \Omega(\log{n})$,
such that solving the problem faster than $q$ rounds requires $q$ bits of advice.

Following the same general approach as with the no-CD case,
assume you can solve the problem with ${\cal A}$ and $f_{\cal A}$, 
in $T$ rounds where $f_{adv}$ gives $x$ bits of advice.

To solve $1$-non-interactive contention resolution with participants $S$, we can provide $f_{\cal A}(S)$
as part of our advice. Assume the nodes running ${\cal A}$ then solve the problem in round $r$.
We could also communicate $r$, as before, but now this is not enough to help the participants
simulate ${\cal A}$ for $r-1$ rounds as they need to know which rounds have collisions.
What we must include in the advice, therefore, is a string of $r-1$ bits,
that indicates for each of those rounds, whether there was a collision ($1$) or not ($0$).
The length of this string implicitly encodes $r$ as well.

The total size of the advice needed to solve $1$-non-interactive contention resolution is therefore upper bounded by $x + r$.
Our algorithm ${\cal A}$ therefore create a contradiction if $x+r < \ell_1$ from Theorem~\ref{thm:noninteractive}.
It follows, therefore, that solve the problem faster than $\ell_1/2 = \Omega(\log{n})$ rounds requires
at last $\ell_1/2$ bits of advice.






% \subsection{An $O(1)$ Round Upper Bound for $O(\log{\log{n}})$ Bits of Advice -- BROKEN}

% {\bf Cal:} {\em Right before the holiday break Alex realized due to some math errors this argument does not work. Indeed there is a lower
% bound that can show it cannot. I have added a new section above to start formalizing this new lower bound and to unfold its implications.}

% \bigskip


% What follows is a deterministic strategy which reduces to $O(1)$ active nodes using $O(\log{\log{n}})$ bits of advice. Generalizing to $O(b)$ bits of advice, the algorithm reduces the number of active nodes to $O\Big(2^{(\log{n}/2^b)}\Big)$. Furthermore, these nodes know the set of possible active nodes after this reduction (and are properly named) and can therefore continue with any existing contention resolution algorithm after this point.

% \par 

% For example, if algorithm $\cal{A}$ takes time $O(\log{n})$ where $n$ is the number of nodes, using this strategy with $O(b)$ bits of advice would have time complexity $O(\log{n}/2^b)$. If $\cal{A}$ instead had time complexity $O(\log{\log{n}})$, the time complexity using $O(b)$ bits of advice would be $O(\log{\log{n}}-b)$.

% \subsubsection{Preliminaries}

% For the analysis that follows, we derive a special case of Stirling's approximation for expressing binomial coefficients that will be useful to our main proof in Lemma \ref{lem:evensplit}.

% \begin{lemma}
% \label{lem:stirlings}

% For integers $\ell$ and $i$ such that $\ell \geq 4$ and $2\leq i\leq \log{\ell}$,
% \[{\ell/2\choose \ell/2^i}\leq 2^\phi\text{ where }\phi=\Bigg(\frac{i-1}{2^{i}}\Bigg)\cdot \ell\]

% \end{lemma}

% \begin{proof}
% By the definition of the binomial coefficient, we have that
% \[{\ell/2\choose \ell/2^i} =\frac{(\ell/2)!}{(\ell/2^i)!\cdot (\ell/2-\ell/2^i)!}\]
% We then apply the Robbins bound of Stirling's approximation to each of the factorials in this expression.
% \begin{align*}
% &\frac{(\ell/2)!}{(\ell/2^i)!\cdot (\ell/2-\ell/2^i)!}\\
% &<E\cdot \frac{\sqrt{2\pi}\cdot (\ell/2)^{\ell/2+1/2}\cdot e^{-\ell/2}}
% {\sqrt{2\pi}\cdot (\ell/2^i)^{\ell/2^i+1/2}\cdot e^{-\ell/2^i}
% \sqrt{2\pi}\cdot (\ell/2-\ell/2^i)^{\ell/2-\ell/2^i+1/2}\cdot e^{-(\ell/2-\ell/2^i)}}
% \\
% % &<\frac{\sqrt{2\pi}\cdot (\ell/2)^{\ell/2+1/2}\cdot e^{-\ell/2}\cdot e^{1/(12\cdot (\ell/2))}}
% % {\sqrt{2\pi}\cdot (\ell/2^i)^{\ell/2^i+1/2}\cdot e^{-\ell/2^i}\cdot e^{1/(12\cdot (\ell/2^i)+1)}
% % \sqrt{2\pi}\cdot (\ell/2-\ell/2^i)^{\ell/2-\ell/2^i+1/2}\cdot e^{-(\ell/2-\ell/2^i)}\cdot e^{1/(12\cdot (\ell/2-\ell/2^i)+1)}
% % }\\
% &=\frac{\sqrt{2\pi}}{2\pi}\cdot E\cdot \frac{e^{\ell/2^i}e^{\ell/2-\ell/2^i}}{e^{\ell/2}}
% \cdot \Bigg(\frac{\ell/2}{(\ell/2^i)\cdot (\ell/2-\ell/2^i)}\Bigg)^{1/2}\cdot \frac{(\ell/2)^{\ell/2}}{(\ell/2^i)^{\ell/2^i}\cdot (\ell/2-\ell/2^i)^{\ell/2-\ell/2^i}}\\
% &\frac{E}{\sqrt{2\pi}}
% \cdot \Bigg(\frac{\ell/2}{(\ell/2^i)\cdot (\ell/2-\ell/2^i)}\Bigg)^{1/2}\cdot \frac{(\ell/2)^{\ell/2}}{(\ell/2^i)^{\ell/2^i}\cdot (\ell/2-\ell/2^i)^{\ell/2-\ell/2^i}}
% \end{align*}
% where
% \begin{align*}
% E&=\frac{e^{1/(12 (\ell/2))}}{e^{1/(12 (\ell/2^i)+1)}\cdot e^{1/(12 (\ell/2-\ell/2^i)+1)}}=\exp{\Bigg(\frac{1}{6\ell}-\frac{1}{12(\ell/2^i)+1}-\frac{1}{12(\ell/2-\ell/2^i)+1}\Bigg)}< \sqrt{\pi}\\
% \end{align*}
% is a bound on the relative error incurred by applying Stirling's approximation (for $\ell\geq 1$). We continue by simplifying the second fraction in our bound,

% \begin{align*}
% \Bigg(\frac{\ell/2}{(\ell/2^i) (\ell/2-\ell/2^i)}\Bigg)^{1/2}
% &=\Bigg(\frac{\ell/2}{(\ell/2^i) (\ell/2-\ell/2^i)}\Bigg)^{1/2}
% =\Bigg(\frac{\ell/2}{(\ell/2^i) (\ell/2) (1-1/2^{i-1})}\Bigg)^{1/2}\\
% &=\Bigg(\frac{1}{(\ell/2^i) (1-1/2^{i-1})}\Bigg)^{1/2}
% =\Bigg(\frac{1}{(\ell/2^i) ((2^{i-1}-1)/2^{i-1}))}\Bigg)^{1/2}\\
% &=\Bigg(\frac{2^i 2^{i-1}}{\ell(2^{i-1}-1)}\Bigg)^{1/2}
% \leq \Bigg(\frac{2^i 2^{i-1}}{2^i(2^{i-1}-1)}\Bigg)^{1/2}
% =\Bigg(\frac{2^{i-1}}{(2^{i-1}-1)}\Bigg)^{1/2}\leq \sqrt{2}
% \end{align*}
% which holds for all $i\geq 2$. Now revisiting our full bound,
% \begin{align*}
% &\frac{E}{\sqrt{2\pi}}
% \cdot \Bigg(\frac{\ell/2}{(\ell/2^i)\cdot (\ell/2-\ell/2^i)}\Bigg)^{1/2}\cdot \frac{(\ell/2)^{\ell/2}}{(\ell/2^i)^{\ell/2^i}\cdot (\ell/2-\ell/2^i)^{\ell/2-\ell/2^i}}\\
% &\leq \frac{\sqrt{\pi}}{\sqrt{2\pi}} \cdot \sqrt{2} \cdot \frac{(\ell/2)^{\ell/2}}{(\ell/2^i)^{\ell/2^i}\cdot (\ell/2-\ell/2^i)^{\ell/2-\ell/2^i}}\\
% &\leq \frac{(\ell/2)^{\ell/2}}{(\ell/2^i)^{\ell/2^i}\cdot (\ell/2-\ell/2^i)^{\ell/2-\ell/2^i}}
% =\frac{(\ell/2)^{\ell/2}}{(\ell/2^i)^{\ell/2^i}\cdot ((\ell/2^i)(2^{i-1}-1))^{(\ell/2^i)(2^{i-1}-1)}}\\
% &=\frac{\ell^{\ell/2}\cdot 2^{i\ell/2^i} \cdot 2^{i(\ell/2^i)(2^{i-1}-1)}}{2^{\ell/2}\cdot \ell^{\ell/2^i}\cdot \ell^{(\ell/2^i)(2^{i-1}-1)}\cdot(2^{i-1}-1)^{(\ell/2^i)(2^{i-1}-1)}}\\
% &=\ell^{\ell/2-\ell/2^i-(\ell/2^i)(2^{i-1}-1)}\cdot \frac{2^{i\ell/2^i} \cdot 2^{i(\ell/2^i)(2^{i-1}-1)}}{2^{\ell/2}\cdot(2^{i-1}-1)^{(\ell/2^i)(2^{i-1}-1)}}
% =\frac{2^{i\ell/2^i} \cdot 2^{i(\ell/2^i)(2^{i-1}-1)}}{2^{\ell/2}\cdot(2^{i-1}-1)^{(\ell/2^i)(2^{i-1}-1)}}
% \end{align*}
% Replacing $2^{i-1}-1$ with $2^{i-1-\varepsilon}$ for some small positive constant $\epsilon\sim 0$, we can express the bound as $2^\phi$ where
% \begin{align*}
%     \phi&=\frac{i\ell}{2^i}+\frac{i\ell (2^{i-1}-1)}{2^i}-\frac{\ell}{2}-(i-1-\varepsilon)\frac{\ell(2^{i-1}-1)}{2^i}
%     =\frac{i\ell}{2^i}-\frac{\ell}{2}+(1+\varepsilon)\frac{\ell(2^{i-1}-1)}{2^i}\\
%     &=\frac{\ell(i-2^{i-1})}{2^i}+(1+\varepsilon)\frac{\ell(2^{i-1}-1)}{2^i}
%     =\ell\cdot \Bigg(\frac{i-2^{i-1}}{2^i}+\frac{2^{i-1}-1}{2^i}+\varepsilon \frac{2^{i-1}-1}{2^i}\Bigg)\\
%     &\leq \ell \cdot \Bigg(\frac{i-1}{2^{i}}+\varepsilon\Bigg)\sim \Bigg(\frac{i-1}{2^{i}}\Bigg)\cdot \ell
% \end{align*}

% \end{proof}
% \subsubsection{Algorithm}

% In the advisor's algorithm, the advisor selects an $\ell$-bit (initially $\ell=\log{n}$) node identifier $u$ from the set of active node identifiers and two-bit string $s\in \{0,1\}^2$ for which $u$ contains at most $\ell/4$ instances of $s$ at even indices. The advisor then removes from the set of active nodes all nodes with $k$ instances of $s$ at even indices where $k> \ell/4$. The advisor renames all active nodes using new $((15/16)\ell)$-bit identifiers and repeats.

% \par

% After $T=O(\log{\log{n}})$ iterations, at most a constant number of active nodes remain. The advisor chooses a constant-bit identifier $u_{T+1}$ from among these. The advisor then sends as advice $\langle s_1,s_2,\ldots,s_T,u_{T+1}\rangle$ where $s_i$ is the value of $s$ chosen in the $i$th iteration of the advisor algorithm.

% \par

% In the candidate algorithm for active node $v$ with an $\ell$-bit identifier and advice $\langle s_1,s_2,\ldots,s_T,u_{T+1}\rangle$, if $v$ contains $k>\ell/4$ instances of the two-bit string $s_1$ (at even indices) it becomes inactive. Each active node $v$ then renames itself using $(15/16)\ell$ bits (based on the set of possible active nodes) and repeats the procedure using $s_2$ and its new identifier length $(15/16)\ell$. After $T$ iterations, if $v=u_{T+1}$ then $v$ broadcasts alone.

% \par

% We begin by introducing a subroutine which heavily leverages the determinism of the algorithm. Given the advice up until a particular iteration, each node knows the set of eligible nodes at this iteration (or at least the subset of all nodes from which the eligible nodes may be drawn). This allows smaller subsets of nodes to perfectly rename themselves using fewer bits.

% \paragraph{Mapping Subroutine}

% Let $S\subseteq \{1,0\}^{b_1}$ be a subset of $b_1$-bit identifiers where $|S|=2^b_2$ for some $b_2<b_1$. If all nodes in $S$ know $S$, they can choose $b_2$-bit identifiers where the identifier of node $v$ is $v$'s position in $S$. Since no two nodes share the same relative position, this mapping is unique.

% \subsubsection{Analysis}

% The first step of our analysis will be to show that for $\ell=\Omega(1)$ and an appropriate choice of $s\in\{0,1\}^2$ in some iteration of the advisor algorithm, the number of eligible $\ell$-bit identifiers is significantly reduced.

% % \begin{algorithm}
% % \SetAlgoNoLine
% % \caption{Rename strings using new number of bits (advisor)}


% % \label{alg:asyncalg}

% % \SetAlgoNoLine

% % \SetKwProg{func}{function}{}{}
% % \SetFuncSty{textsc}

% % \SetKwFunction{rename}{Rename}
% % \func{\rename{$A$}}
% % {

% % $\ell_{new}\gets \log{|A|}$\;
% % $A_{new}\gets\emptyset$\;
% % $M\gets [:]\;$

% % \For{$a\in A$}
% % {
% %     $i_a\gets a\text{'s relative rank in }A$\;
% %     $A_{new}\gets A_{new}\cup \{i_a\}$\;
% %     $M[i_a]\gets a$;
% % }

% % \Return $\langle A_{new}, \ell_{new}, M\rangle$
% % }
% % \end{algorithm}



% % \begin{algorithm}
% % \SetAlgoNoLine
% % \caption{Remove instances of substring {\tt '00'} from all strings (advisor)}


% % \label{alg:asyncalg}

% % \SetAlgoNoLine

% % \SetKwProg{func}{function}{}{}
% % \SetFuncSty{textsc}

% % \SetKwFunction{zero}{00-Erase}
% % \func{\zero{$A, \ell$}}
% % {

% % k=0\;
% % \While{$\text{for all }a\in A\text{ there exists some }i\in \ell/2\text{ s.t. }a[2i,2i+1]={\tt '00'}$}
% % {
% % \For{$a\in A$}
% % {
% %     (replace first instance of {\tt '00'} in $A$ with $\epsilon$)\;
% %     $\ell \gets \ell - 2$\;
% %     $k \gets k + 1$\;
% % }
% % }
% % \Return $\langle A, \ell\rangle$
% % }
% % \end{algorithm}



% % \begin{algorithm}
% % \SetAlgoNoLine
% % \caption{Selection algorithm (advisor)}

% % \label{alg:asyncalg}

% % \SetAlgoNoLine

% % \SetKwProg{func}{function}{}{}
% % \SetFuncSty{textsc}

% % \SetKwFunction{select}{AdvisorSelect}
% % \func{\select{$A, \ell$, k}}
% % {

% % $\langle A', \ell', k\rangle \gets \textsc{00-Erase}(A,\ell)$\;
% % \If{$k\leq \ell/32$}
% % {
% % \Return $\textsc{AdvisorSelect}(\textsc{Rename}(A, (3/4)\cdot \ell), (3/4)\cdot \ell, k)$
% % }
% % \Else
% % {

% % }

% % \While{$\text{for all }a\in A\text{ there exists some }i\in \ell/2\text{ s.t. }a[2i,2i+1]={\tt '00'}$}
% % {
% % \For{$a\in A$}
% % {
% %     (replace first instance of {\tt '00'} in $A$ with $\epsilon$)\;
% %     $\ell \gets \ell - 2$\;
% %     $k \gets k + 1$\;
% % }
% % }



% \begin{lemma}
% \label{lem:evensplit}

% Fix a two-bit substring $s\in \{0,1\}^2$ and length $64\leq \ell\leq \log{n}$. For any $k\in [\ell/4]$, the number of possible strings with at most $k$ instances of $s$ at even indices is at most $2^{(15/16)\ell}$.
% \end{lemma}
% \begin{proof}

% For any $k$ and two-bit string $s$, the number of ways that exactly $k$ instances of $s$ can be placed in an $\ell$-bit string at even indices is at most ${\ell/2 \choose k}$. Furthermore, given that there are no more instances of $s$ at even indices, the remaining two-bit substrings at even indices must belong to $\Sigma=\{0,1\}^2\setminus\{s\}$. Lastly, since there are $\ell-2 k$ remaining bits (and therefore $(\ell-2 k)/2$ remaining even indices) and $|\Sigma|=3$, there are at most $3^{\frac{1}{2}(\ell-2k)}$ ways to choose the remaining bits. Therefore, the number of potential strings with exactly $k$ instances of $s$ at even indices is at most
% \[{\ell/2 \choose k}\cdot 3^{\frac{1}{2}(\ell-2k)}\]
% Next, since $k\leq \ell / 4$, we can set $k=\ell/2^i$ and apply Lemma \ref{lem:stirlings} to simplify the binomial coefficient.

% \begin{align*}
%     {\ell/2 \choose k}\cdot 3^{\frac{1}{2}(\ell-2k)}
%     &={\ell/2 \choose \ell/2^i}\cdot 3^{\frac{1}{2}(\ell-2\cdot(\ell/2^i))}
%     \leq 2^{((i-1)/2^i)\cdot \ell}\cdot 3^{\frac{1}{2}(\ell-2\cdot(\ell/2^i))}\\
%     &\leq 2^{((i-1)/2^i)\cdot \ell}\cdot \Big(2^{8/5}\Big)^{\frac{1}{2}(\ell-2\cdot(\ell/2^i))}
%     =2^{((i-1)/2^i)\cdot \ell}\cdot 2^{\frac{4}{5}(\ell-2\cdot(\ell/2^i))}=2^\phi\\
% \end{align*}

% We now demonstrate that $2^\phi<2^{(7/8)\ell}$, by verifying that $\phi<\frac{7}{8}\ell$ for $i\geq 2$. This is a stronger bound than required by our Lemma but recall this bound still only considers strings with \emph{exactly} $k$ instances of $s$.

% \begin{align*}
%     \phi=\ell \frac{i-1}{2^i}+\ell \frac{4}{5} \Bigg(1-\frac{1}{2^{i-1}}\Bigg)&< \frac{7}{8} \ell\\
%     \frac{i-1}{2^i}+ \frac{4}{5} \Bigg(1-\frac{1}{2^{i-1}}\Bigg)&< \frac{7}{8} \\
%     \frac{i-1}{2^i}+ \frac{4}{5}- \frac{4}{5}\frac{1}{ 2^{i-1}}&< \frac{7}{8} \\
%     i-1+\frac{4}{5} 2^i -\frac{8}{5}&<\frac{7}{8}  2^i\\
%     i-\frac{13}{5}&<\bigg(\frac{7}{8} -\frac{4}{5}\bigg)\cdot2^i \\
%     i-\frac{13}{5}&<\frac{3}{40}2^i\\
%   40i&<3\cdot 2^i+104\\
% \end{align*}

% % Since $k\leq \ell/4$ (and so $i\geq 2$), the above is satisfied for all values of $i$ assumed by the Lemma.
% Now we can upper bound the number of strings with \textit{at most} $k$ instances of $s$. This is due to the fact that our bound holds for all $k\leq \ell/4$ and so it also applies to each value $k'\leq k$.

% \begin{align*}
%     \sum_{k'=1}^{k}2^{(7/8)\ell}
%     \leq \sum_{k'=1}^{\ell/4}2^{(7/8)\ell}
%     = \frac{\ell}{4}2^{(7/8)\ell}
%     = 2^{\log{\ell}-2}\cdot 2^{(7/8)\ell}
%     = 2^{(7/8)\ell+\log{\ell}-2}
%     \leq 2^{(15/16)\ell}
% \end{align*}

% Where the last inequality holds for any $\ell$ such that $\ell/16\geq \log{\ell}-2$ (eg. $\ell \geq 64$).

% \end{proof}

% From the above, we have that by requiring all eligible $\ell$-bit identifiers to have at most $\ell/4$ instances of some two-bit substring $s\in \{0,1\}^2$, we eliminate all but at most $2^{(15/16)\cdot \ell}$ identifiers. This allows us to rename the remaining nodes with $O((15/16)\ell)$ bits.

% \par

% Furthermore, since $s$ and $k$ are chosen with an identifier in mind, this set of identifiers is always nonempty, however this statement needs an assurance that in any iteration there is some $\ell$-bit identifier with at most $\ell/4$ occurrences of \textit{some} two-bit string at even indices. However, this holds trivially for any value of $\ell$ for some $s$ since if each two-bit substring appears more than $\ell/4$ times then the number of bits would be larger than $2\ell>\ell$.

% \paragraph{Bit Complexity of Advice} By applying $T=O(\log{\log{n}})$ iterations of the algorithm (as long as $\ell=\Omega(1)$), the number of nodes which remain active is given by
% \[\Bigg(\Big(2^{\log{n}}\Big)^{(15/16)}\Bigg)^T=\Bigg(\Big(2^{\log{n}}\Big)^{(15/16)}\Bigg)^{O(\log{\log{n}})}=\Big(2^{\log{n}}\Big)^{O(\log^{-1}{n})}=2^{O(1)}\]

% At this point, the final node can then be identified with at most $O(1)$ bits. Since there are at most $O(\log{\log{n}})$ iterations and for any iteration $i$ the choice of $s_i$ is $O(1)$ bits, the total bit complexity of the advice string is
% $O(\log{\log{n}})$ bits. If instead only $O(b)<O(\log\log{n})$ bits of advice are allowed, the number of remaining active nodes is instead generalized to

% \[\Bigg(\Big(2^{\log{n}}\Big)^{(15/16)}\Bigg)^b=\Big(2^{\log{n}}\Big)^{O(2^{-b})}=2^{O(\phi)}\text{ where }\phi =\frac{\log{n}}{{2^b}}\]


% \begin{align*}
%     &(i-1)\cdot \Bigg[2^{i-1}\cdot \Bigg(\frac{\ell}{2^i} -1\Bigg) +1\Bigg] - (i-1-\varepsilon)\cdot (2^{i-1}-1)\cdot \Bigg(\frac{\ell}{2^i}-1\Bigg)\\
%     &=(i-1)\cdot \Bigg(\frac{\ell}{2} -2^{i-1} +1\Bigg) - (i-1-\varepsilon)\cdot \Bigg(\frac{\ell}{2}-2^{i-1}-\frac{\ell}{2^i}+1\Bigg)\\
%     &=i\cdot \Bigg(\frac{\ell}{2} -2^{i-1} +1\Bigg) - \Bigg(\frac{\ell}{2} -2^{i-1} +1\Bigg) - i \cdot \Bigg(\frac{\ell}{2}-2^{i-1}-\frac{\ell}{2^i}+1\Bigg)+(1+\varepsilon)\cdot \Bigg(\frac{\ell}{2}-2^{i-1}-\frac{\ell}{2^i}+1\Bigg)\\
%     &=\ell\cdot \frac{i}{2^i} - \Bigg(\frac{\ell}{2} -2^{i-1} +1\Bigg) +(1+\varepsilon)\cdot \Bigg(\frac{\ell}{2}-2^{i-1}-\frac{\ell}{2^i}+1\Bigg)\\
%     &=\ell\cdot \frac{i}{2^i} - (1+\varepsilon)\cdot \frac{\ell}{2^i} + \varepsilon\cdot \Bigg(\frac{\ell}{2}-2^{i-1}-\frac{\ell}{2^i}+1\Bigg)\\
% \end{align*}


\subsection{An $\Omega(\log\log{n}- b)$ Round Lower Bound for $b$ Bits of Advice, Constant Probability, and CD}

Let us now consider the case with collision detection with constant probability.
In the no advice setting, Willard's algorithm solves the problem
in $O(\log\log{n})$ rounds for these assumptions, by essentially
performing a binary search through the $\log{n}$ different possible
size classes for the participants (1,2,4,...,n),
using a collision as an indication that your guess is too small,
and silence as an indication that your guess is too large.
On arriving at a good guess, then as argued earlier for constant probability and no CD,
a constant number of additional broadcasts can drive the failure probability below $1/2$.

From the lower bound perspective,
the no advice lower bound paper demonstrated this bound to be tight through a simulation argument.
Assume you could solve this problem with constant probability in $t=o(\log\log{n})$ rounds with CD.
We then use this to solve the problem with constant probability in $2^t = o(\log{n})$ rounds
with {\em no} CD. 
The trick is to run a $t$ round simulation of the original algorithm again and again, each time making
different guesses at what the collision detector should return. 
There are $2^t$ possible sequences of collision detector responses.
One of them will be right.
In the simulation with those guesses, the protocol works.
(A small technicality is that we must use the same randomness locally in each simulation).

I do not see any obstacle to applying this same strategy to the setting in which we also allow advice.
If you can solve the problem in $t$ rounds with collision detection and advice,
we can solve the problem with the same probability in $2^t$ rounds with no collision detection and advice.
This becomes trouble when $2^t \leq (c\log{n}/2^b)$ for the constant $c$ specified by the relevant no collision detection lower bound.
So we get $t \leq \log((c\log{n}/2^b)) = O(\log\log{n}) - b$ as the bound.

\begin{theorem}
Let ${\cal A}$ be a $b$-advice protocol,
for some $b \geq 0$,
that guarantees for every $n>1$ and collision detection,
to solve contention resolution in at most $t_b(n)$ rounds with probability at least $1/2$.
It follows:

\[ t_b(n) \in \Omega\left(\log\log{n}\right) - b. \]
\end{theorem}

\paragraph{Notes on a Matching Upper Bound.}
I believe that Willard's strategy should adapt to match this bound.
Assume that the advice function uses its $b$ bits to narrow down the range of
size classes to test from $\log{n}$ to $\log{n}/2^b$.
Now when we run the Willard strategy of performing a binary search
over the possible size classes, 
this search focuses on only $\log{n}/2^b$ classes,
requiring $\log\left( \frac{\log{n}}{2^b} \right) = \log\log{n} - b$ steps.



\subsection{A Vastly Simpler Way to Prove 3 out of 4 of the Above Lower Bounds}

As I was finishing up my summary of the above lower bounds it struck me
that there is a vastly simpler, black box argument for advice bounds that matches 3 out of
4 bounds established above.
The simple idea is that $b$ bits cannot speed things up by more than a factor of $2^b$,
as if it did, you could guess the advice, and one of your $2^b$ guesses would be correct.
This approach, formalized below, gives us the same bound as established above,
with the exception of constant probability with collision detection.
For that final case, our above argument provides an even stronger bound.

\begin{theorem}
Assume no algorithm can guarantee to solve contention resolution in less than $t_{opt}(n)$ rounds with
probability at least $p$ for a given assumption about whether or not collision detection is available.
Let ${\cal A}$ be a $b$-advice algorithm that solves contention resolution in $t_b(n)$ rounds with probability
at least $p$ and the same collision detection assumption.
It follows: \[ t_b(n) \geq t_{opt}(n)/2^b. \]

\end{theorem}
\begin{proof}
Fix some $t_{opt}(n)$, $p$,and collision detection assumption, as specified in the theorem statement.
Assume some $b$-advice algorithm ${\cal A}$ can solve the problem in less than $t_{opt}(n)/2^b$
rounds with this same probability and collision detection assumption.
We use ${\cal A}$ to construct an algorithm ${\cal A'}$ that does not use
advice.
This new algorithm runs $2^b$ simulations of ${\cal A}$, one for each of the possible
advice strings of length $b$ it might obtain from an advice function.
The simulation corresponding to the correct guess for the given set of participants
will solve the problem with probability at least $p$ after it has been simulated for
strictly less than $t_{opt}(n)/2^b$ rounds which corresponds to strictly less than $t_{opt}(n)$
total rounds---contradiction the optimally of $t_{opt}$.

\end{proof}
